MAP Estimators for Piecewise Continuous Inversion

We study the inverse problem of estimating a field $u$ from data comprising a finite set of nonlinear functionals of $u$, subject to additive noise; we denote this observed data by $y$. Our interest is in the reconstruction of piecewise continuous fields in which the discontinuity set is described by a finite number of geometric parameters. Natural applications include groundwater flow and electrical impedance tomography. We take a Bayesian approach, placing a prior distribution on $u$ and determining the conditional distribution on $u$ given the data $y$. It is then natural to study maximum a posterior (MAP) estimators. Recently (Dashti et al 2013) it has been shown that MAP estimators can be characterised as minimisers of a generalised Onsager-Machlup functional, in the case where the prior measure is a Gaussian random field. We extend this theory to a more general class of prior distributions which allows for piecewise continuous fields. Specifically, the prior field is assumed to be piecewise Gaussian with random interfaces between the different Gaussians defined by a finite number of parameters. We also make connections with recent work on MAP estimators for linear problems and possibly non-Gaussian priors (Helin, Burger 2015) which employs the notion of Fomin derivative. In showing applicability of our theory we focus on the groundwater flow and EIT models, though the theory holds more generally. Numerical experiments are implemented for the groundwater flow model, demonstrating the feasibility of determining MAP estimators for these piecewise continuous models, but also that the geometric formulation can lead to multiple nearby (local) MAP estimators. We relate these MAP estimators to the behaviour of output from MCMC samples of the posterior, obtained using a state-of-the-art function space Metropolis-Hastings method.

==> references <==
\begin{thebibliography}{10}

\bibitem{hitchhiker}
C.~D. Aliprantis and K. Border.
\newblock {\em {Infinite Dimensional Analysis: A Hitchhiker's Guide}}.
\newblock 2007.

\bibitem{largescale}
L. Biegler, G. Biros, O. Ghattas, M. Heinkenschloss, D. Keyes, B. Mallick, L.
  Tenorio, B. van Bloemen~Waanders, K. Willcox, and Y. Marzouk.
\newblock {\em Large-scale inverse problems and quantification of uncertainty},
  volume 712.
\newblock John Wiley \& Sons, 2011.

\bibitem{bogachev-fomin}
V.~I. Bogachev.
\newblock {Differentiable measures and the Malliavin calculus}.
\newblock {\em Journal of Mathematical Sciences}, 87(4):3577--3731, 1997.

\bibitem{besovmap}
T. Bui-Thanh and O. Ghattas.
\newblock {A Scalable MAP Solver for Bayesian Inverse Problems with Besov
  Priors}.
\newblock 9(November):27--53, 2012.

\bibitem{historymatching}
J. Carter and D. White.
\newblock History matching on the imperial college fault model using parallel
  tempering.
\newblock {\em Computational Geosciences}, 17(1):43--65, 2013.

\bibitem{pcn}
S.~L. Cotter, G.~O. Roberts, A.~M. Stuart, and D. White.
\newblock {MCMC methods for functions modifying old algorithms to make them
  faster}.
\newblock {\em Statistical Science}, 28(3):424--446, 2013.

\bibitem{dacorogna}
B. Dacorogna.
\newblock {\em {Direct methods in the calculus of variations}}.
\newblock Springer, 2008.

\bibitem{darcy}
H. Darcy.
\newblock {\em {Les fontaines publiques de la ville de Dijon}}.
\newblock 1856.

\bibitem{map}
M. Dashti, K.~J.~H. Law, A.~M. Stuart, and J. Voss.
\newblock {MAP estimators and their consistency in Bayesian nonparametric
  inverse problems}.
\newblock {\em Inverse Problems}, 29(9):095017, 2013.

\bibitem{lecturenotes}
M. Dashti and A.~M. Stuart.
\newblock {The Bayesian Approach to Inverse Problems}.
\newblock {\em arXiv:1302.6989v3}.

\bibitem{eit}
M.~M. Dunlop and A.~M. Stuart.
\newblock {The Bayesian Formulation of EIT: Analysis and Algorithms}.
\newblock {\em arXiv:1508.04106}, 2015.

\bibitem{linear1}
J.~N. Franklin.
\newblock {Well posed stochastic extensions of ill posed linear problems}.
\newblock {\em Journal of Mathematical Analysis and Applications},
  31(3):682--716, 1970.

\bibitem{gilbarg}
D. Gilbarg and N.~S. Trudinger.
\newblock {\em Elliptic partial differential equations of second order}.
\newblock Springer, 2015.

\bibitem{wmap}
T. Helin and M. Burger.
\newblock {Maximum a posteriori probability estimates in infinite-dimensional
  Bayesian inverse problems}.
\newblock {\em Inverse Problems}, 31(8):085009, 2015.

\bibitem{eit78}
R.~P. Henderson and J.~G. Webster.
\newblock {An impedance camera for spatially specific measurements of the
  thorax}.
\newblock {\em IEEE transactions on bio-medical engineering}, 25(3):250--254,
  1978.

\bibitem{kui}
M.~A. Iglesias, K. Lin, and A.~M. Stuart.
\newblock {Well-Posed Bayesian Geometric Inverse Problems Arising in Subsurface
  Flow}.
\newblock {\em Inverse Problems}, 30, 2014.

\bibitem{frechet}
J.~P. Kaipio, V. Kolehmainen, E. Somersalo, and M. Vauhkonen.
\newblock {Statistical inversion and Monte Carlo sampling methods in electrical
  impedance tomography}.
\newblock {\em Inverse Problems}, 16(5):1487--1522, 2000.

\bibitem{kaipio}
J.~P. Kaipio and E. Somersalo.
\newblock {\em {Statistical and Computational Inverse Problems}}.
\newblock Springer, 2005.

\bibitem{kinder}
D. Kinderlehrer and G. Stampacchia.
\newblock {\em {An introduction to variational inequalities and their
  applications}}, volume~31.
\newblock 1980.

\bibitem{ert33}
R.~E. Langer.
\newblock {An inverse problem in differential equations}.
\newblock {\em Bulletin of the American Mathematical Society}, 39(10):814--821,
  1933.

\bibitem{lasanen1}
S. Lasanen.
\newblock {Non-Gaussian Statistical Inverse Problems. Part I: Posterior
  Distributions}.
\newblock {\em Inverse Problems \& Imaging}, 6(2), 2012.

\bibitem{lasanen2}
S. Lasanen.
\newblock {Non-Gaussian Statistical Inverse Problems. Part II: Posterior
  Convergence for Approximated Unknowns}.
\newblock {\em Inverse Problems \& Imaging}, 6(2), 2012.

\bibitem{besovprior}
M. Lassas, E. Saksman, and S. Siltanen.
\newblock Discretization-invariant {B}ayesian inversion and {B}esov space
  priors.
\newblock {\em Inverse Problems and Imaging}, 3, 2009.

\bibitem{point_est}
E.~L. Lehmann and G. Casella.
\newblock {\em {Theory of Point Estimation}}.
\newblock 1998.

\bibitem{linear2}
M.~S. Lehtinen, L. Paivarinta, and E. Somersalo.
\newblock {Linear inverse problems for generalised random variables}.
\newblock {\em Inverse Problems}, 5(4):599--612, 1999.

\bibitem{lifshits}
M.~A. Lifshits.
\newblock {\em Gaussian random functions}, volume 322.
\newblock Springer, 1995.

\bibitem{linear3}
A. Mandelbaum.
\newblock {Linear estimators and measurable linear transformations on a Hilbert
  space}.
\newblock {\em Zeitschrift f\"{u}r Wahrscheinlichkeitstheorie und Verwandte
  Gebiete}, 65(3):385--397, 1984.

\bibitem{uniqueness_median}
P. Milasevic and G.~R. Ducharme.
\newblock {Uniqueness of the Spatial Median}.
\newblock {\em Annals of Statistics}, 15(3):1332--1333, 1987.

\bibitem{NF98}
G.~K. Nicholls and C. Fox.
\newblock Prior modelling and posterior sampling in impedance imaging.
\newblock In A. Mohammad-Djafari, editor, {\em Bayesian Inference for Inverse
  Problems}, volume 3459, pages 116--127. SPIE, 1998.

\bibitem{nocedal}
J. Nocedal and S. Wright.
\newblock {\em Numerical optimization}.
\newblock Springer Science \& Business Media, 2006.

\bibitem{reservoir}
D. Oliver, A. Reynolds, and N. Liu.
\newblock {\em {Inverse Theory for Petroleum Reservoir Characterization}}.
\newblock Cambridge University Press, 2008.

\bibitem{cheney}
E. Somersalo, M. Cheney, and D. Isaacson.
\newblock {Existence and Uniqueness for Electrode Models for Electric Current
  Computed Tomography}.
\newblock {\em SIAM Journal on Applied Mathematics}, 52(4):1023--1040, 1992.

\bibitem{inverse}
A.~M. Stuart.
\newblock {Inverse problems : a Bayesian perspective}.
\newblock {\em Acta Numerica}, 19(May 2010):451--559, 2010.

\bibitem{sidak}
Z. \v{S}id\'{a}k.
\newblock {On multivariate normal probabilities of rectangles: their dependence
  on correlations}.
\newblock {\em The Annals of Mathematical Statistics}, pages 1425--1434, 1968.

\end{thebibliography}

